Evaluating Weakly Supervised Object Localization Methods Right

Weakly-supervised object localization (WSOL) has gained popularity over the last years for its promise to train localization models with only image-level labels. Since the seminal WSOL work of class activation mapping (CAM), the field has focused on how to expand the attention regions to cover objects more broadly and localize them better. However, these strategies rely on full localization supervision to validate hyperparameters and for model selection, which is in principle prohibited under the WSOL setup. In this paper, we argue that WSOL task is ill-posed with only image-level labels, and propose a new evaluation protocol where full supervision is limited to only a small held-out set not overlapping with the test set. We observe that, under our protocol, the five most recent WSOL methods have not made a major improvement over the CAM baseline. Moreover, we report that existing WSOL methods have not reached the few-shot learning baseline, where the full-supervision at validation time is used for model training instead. Based on our findings, we discuss some future directions for WSOL.

==> trash.tex <==

\if 0 
The aim of the WSOL task is to produce a scoring function $s_{ij}:=s(X_{ij})$ such that thresholding it at $\tau$ closely approximates the ground truth pixel-wise mask: $1_{s_{ij}\geq\tau}\approx T_{ij}$.
We illustrate the overview of this inference time procedure in Figure~\ref{fig:overview}.
Many existing approaches for WSOL, including CAM~\cite{CAM} and its variants, use scoring rules based on the pixel-wise posterior $s_{ij}=p(Y|X_{ij})$. See Appendix for the interpretation of CAM as pixel-wise posterior approximation.

\subsection{When is WSOL ill-posed?}
\label{subsec:when_is_wsol_unsolvable}

We show that when some background cues are more strongly associated with the target labels than some foreground cues, even if we have certain oracle information on $p(Y|X_{ij})$, the localization task $p(T_{ij}| X_{ij})$ cannot be solved. We will first make several strong assumptions in favor of the learner, and then show that WSOL still cannot be solved perfectly depending on the data distribution. 

For a scoring rule $s$ and a threshold $\tau$, we define the \textbf{pixel-wise localization accuracy} $\text{\pxacc}(s,\tau)$ as the probability of correctly predicting the pixel-wise labels:
\begin{align}
    \text{\pxacc}(s,\tau)=
    {P}_{X,T}(s_{ij}\geq\tau\mid T_{ij}=1)\cdot{P}_{X,T}(T_{ij}=1)
    \nonumber\\
    +{P}_{X,T}(s_{ij}<\tau\mid T_{ij}=0)\cdot{P}_{X,T}(T_{ij}=0)
    \nonumber
\end{align}

To make the analysis easier, we introduce the concept of \textbf{cues}. For example, given an image of a duck, present cues may either be fine-grained foreground object cues like \{duck's head, duck's feet\} or background cues like \{sky, lake\}. 

\newcommand{\eqd}{\text{duck}}
\newcommand{\eqnd}{\text{duck}^c}
\newcommand{\eqf}{\text{feet}}
\newcommand{\eql}{\text{lake}}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/wsol_illposed.pdf}
    \caption{\small\textbf{Ill-posed WSOL: An example.} Even if we have correct cue labels $M$ (an oracle cue detector) and true posteriors $p(Y|M)$ (an oracle image patch classifier), a CAM-based WSOL method will fail to localize feet correctly if $p(\eql|\eqd)\gg p(\eqf|\eqd)$.}
    \label{fig:duck_feet_lake}
\end{figure}

One common simplifying assumption is that each image patch can be fully represented by the cue label. Specifically, there exists a deterministic function $M$ that maps every image patch to a single cue label $M_{ij}:=M(X_{ij})\in\mathcal{M}$. We further assume that the patch score depends on the image patch $s(X_{ij})$ only through the cue label $M_{ij}$; \ie, $s(X_{ij})=s(M_{ij})$. Finally, every cue label is deterministically mapped by $T$ to the binary presence label $T(\cdot)\in\{0,1\}$, \eg $T(\text{duck's feet})=1$ and $T(\text{lake})=0$. Assuming the perfect cue detector $X_{ij}\mapsto M_{ij}$, the localization task then boils down to the estimation of $T(M_{ij})$ for the given cue label $M_{ij}$. 

As indicated by the lemma, even with the full knowledge on the joint distribution of image-level labels and cue labels $p(Y,M)$, it may not be possible to obtain the perfect pixel-wise labeling $T(M)$ (see Appendix for the proof).
\begin{lemma}
    Assume that the true posterior $p(Y|M)$ with the continuous pdf is used as the scoring rule $s(M)=p(Y| M)$. Then, there exists a scalar $\tau\in \mathbb{R}$ such that $\text{\pxacc}(p(Y| M),\tau)=1$ if and only if the foreground-background posterior ratio $\frac{p(Y=1| M)}{p(Y=1| M^\prime)}\geq 1$ almost surely, conditionally on the event $E:=\{T(M)=1\text{ and }T(M^\prime)=0\}$.
\end{lemma}
Intuitively, {if the posterior likelihood for $Y$ given a foreground cue $M$ is less than the posterior likelihood given background $M^\prime$ with non-zero probability, the WSOL cannot make a correct prediction}. This pathological scenario is observed when $\alpha<1$ which arises in real data
when (1) the foreground likelihood ratios ${p(M| Y=1)}/{p(M^\prime|Y=1)}$ are low (Figure~\ref{fig:duck_feet_lake} for example), or (2) the background likelihood ratios ${p(M| Y=0)}/{p(M^\prime | Y=0)}$ are high. This observation implies a data-centric solution towards well-posed WSOL: we can augment (1) positive samples ($Y=1$) with more less-represented foreground cues (\eg $M=\text{duck's feet}$) and (2) negative samples ($Y=0$) with more target-correlated background cues (\eg  $M^\prime=\text{lake}$). Such data-centric approaches are promising future research directions for turning WSOL into a well-posed task. In this paper, however, we remark that previous WSOL methods have relied on implicit full supervision and focus on addressing ill-posedness of WSOL through a small held-out set of fully supervised samples.
\fi
